FedBEVT: Federated Learning Bird's Eye View Perception Transformer in Road Traffic Systems

Bird's eye view (BEV) perception is becoming increasingly important in the field of autonomous driving. It uses multi-view camera data to learn a transformer model that directly projects the perception of the road environment onto the BEV perspective. However, training a transformer model often requires a large amount of data, and as camera data for road traffic are often private, they are typically not shared. Federated learning offers a solution that enables clients to collaborate and train models without exchanging data but model parameters. In this paper, we introduce FedBEVT, a federated transformer learning approach for BEV perception. In order to address two common data heterogeneity issues in FedBEVT: (i) diverse sensor poses, and (ii) varying sensor numbers in perception systems, we propose two approaches -- Federated Learning with Camera-Attentive Personalization (FedCaP) and Adaptive Multi-Camera Masking (AMCM), respectively. To evaluate our method in real-world settings, we create a dataset consisting of four typical federated use cases. Our findings suggest that FedBEVT outperforms the baseline approaches in all four use cases, demonstrating the potential of our approach for improving BEV perception in autonomous driving.

==> sections/07_dataset.tex <==
\section{Details on FedBEVT Dataset}


\begin{figure*}[!ht]
   \centering   \includegraphics[width=1\textwidth]{figures/FedBEVT_Dataset.png}
   \caption{Distribution of federated dataset for evaluation of the FedBEVT in UC~1-4.}
   \label{fig:data}
\end{figure*}

\setlength{\tabcolsep}{3pt}
\begin{table*}[h!]
\centering
\fontsize{8}{12}\selectfont
%\bgroup\footnotesize
\begin{threeparttable}
\caption{Sensor configuration parameters used for data
collection in car, bus ,truck and infrastructure clients.}
\label{table:data_sensor}
\begin{tabular}{C{1.7cm}|C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}|C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}|C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}|C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}}
\toprule %%%%%%%%%%%%%%%%%%
\multirow{1}{*}{Veh. Type} &\multicolumn{4}{c|}{Car} & \multicolumn{4}{c|}{Bus} & \multicolumn{4}{c|}{Truck}  & \multicolumn{4}{c}{Infrastructure}\\
% \cmidrule(lr{0em}){2-10}
Sensor ID & Front & Left & Right &  Rear & Front & Left & Right &  Rear & Front & Left & Right &  Rear & Front & Left & Right &  Rear\\
\midrule
\midrule
Roll (degree) &  0 &  0&  0&  0 & 0 &0  & 0 & 0  & 0 & 0 & 0 & 0  &0  & 0 & 0 & 0  \\
Pitch (degree) &  0&  0&  0&  0&  -5&  -5&  -5&   -5&  -5&  -5&  -5&  -5 & -10 & -10 & -10 & -10 \\
Yaw (degree)&  0& 100 & -100 & 180  & 0  & 100 & -100 & 180   & 0 & 100 & -100 & 180   & 0 &  100 & -100 & 180 \\
Height (m)&  1.8&  1.8&  1.8&   1.8&  3.2&  3.2&  3.2&   3.2&  4.8&  4.8&  4.8&   4.8&  8.2& 8.2 & 8.2 & 8.2 \\
\bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\end{threeparttable}
\end{table*}


\begin{figure*}[!ht]
   \centering   \includegraphics[width=1\textwidth]{figures/fedbevt_pose_variation_v2.png}
   \caption{Visualization of four-view camera data points and BEV groundtruth (GT) for car, bus, truck, and infrastructure clients in the FedBEVT dataset. }
   \label{fig:pose_variation}
\end{figure*}

\begin{figure*}[!ht]
   \centering   \includegraphics[width=1\textwidth]{figures/fedbevt_other_variations_v2.png}
   \caption{Further visualization of four-view camera data points for additional data variation types of varying weather and light conditions.}
   \label{fig:additional_variations}
\end{figure*}

\setlength{\tabcolsep}{3pt}
\begin{table}[h!]
\centering
\fontsize{9}{12}\selectfont
%\bgroup\footnotesize
\begin{threeparttable}
\caption{Overview of the underlying data heterogeneity causes in federated learning for road environmental perception. Four categories of general data variation types can be identified, which include feature distribution skew (FDS), label distribution skew (LDS), covariate skew (CS) and quantity skew (QS).}
\label{table:data_variation}
\begin{tabular}{C{3cm}|C{1cm}C{1cm}C{1cm}C{1cm}}
\toprule %%%%%%%%%%%%%%%%%%
\multirow{1}{*}{Data Variation Type} &\multicolumn{1}{c|}{FDS} & \multicolumn{1}{c|}{LDS} & \multicolumn{1}{c|}{CS} & \multicolumn{1}{c}{QS}\\
% \cmidrule(lr{0em}){2-10}
\midrule
\midrule
\textbf{Sensor pose} & \checkmark  &  - & - & -\\
\textbf{Sensor number} & \checkmark  & - & - & -\\
\midrule
Sensor type & \checkmark  & - & \checkmark & -\\
Scenario & \checkmark  & \checkmark & \checkmark & -\\
Weather & \checkmark  & - & - & - \\
Light condition & \checkmark  & - & - & - \\
Number of vehicles  &-  & -  & - & \checkmark\\
Test kilometers  &-  & -  & - & \checkmark\\
\bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\end{threeparttable}
\end{table}


First, we provide the distribution of data among clients for the four UCs used in the evaluation in Fig.~\ref{fig:data}. Except for UC~4, which contains only car data, each UC contains data collected by bus and truck sensor systems.

In Tab.~\ref{table:data_sensor}, we report the sensor configuration parameters used for data
collection in car, bus, truck and infrastructure clients. We qualitatively show the difference of input multi-camera data among bus, truck and car clients in Fig.~\ref{fig:pose_variation}. 

One of the main challenges in obtaining a federated learning dataset is identifying the Non-IID data distribution among clients based on their realistic scenarios and allocating the data in a more meaningful way among clients. Many publicly available federated learning datasets~\cite{hu2022oarf, caldas2018leaf} are often made based on toy datasets. While these datasets are significant for benchmarking and validating the general properties of federated learning algorithms~\cite{li2022federated}, they may not be suitable for evaluating algorithm performance on more specific applications or tasks such as environmental perception for autonomous driving~\cite{9857660,9982368, 9013081}. Therefore, it is crucial to create and use more realistic and diverse datasets that reflect the complexities of real-world scenarios. 
The current datasets available for multi-camera data in road traffic systems, including KITTI~\cite{Geiger2012CVPR}, nuScenes~\cite{caesar2020nuscenes}, and OPV2V~\cite{xu2022opv2v}, are not designed for federated learning studies. While prior research~\cite{9564384} has explored federated object detection by distributing existing datasets among multiple clients, the heterogeneity of the data captured by different camera systems cannot be addressed, as each of these datasets is collected using the same camera setup. The dataset proposed by Luo et al.~\cite{luo2019real} is specifically designed for federated learning. However, it only addresses label distribution skew, and also is unsuitable for tasks involving multi-view camera data or BEV perception.
In this context, we create the \textbf{first federated dataset for BEV perception tasks}, which is also \textbf{the first dataset that takes into account the various camera configurations among clients}, a common occurrence in real-world federated learning scenarios of road traffic systems.

In addition, we classify the two addressed types of data variations: (\emph{i}) diverse sensor poses, and (\emph{ii}) varying sensor numbers, into the general categories of data variations in federated learning~\cite{kairouz2021advances}, as outlined in Table~\ref{table:data_variation}. Both sensor pose and number can cause feature distribution skew, where different distribution of input features (as shown in~\ref{fig:pose_variation}) can be mapped to the same labels. However, previous work~\cite{9564384, 9827020, yu2019federated} has primarily focused on addressing label distribution skew and quantity skew, which are less common in BEV perception tasks. As an analysis results, we list other possible data variations types also in Tab.~\ref{table:data_variation}.

Finally, we introduce futher dataset for FedBEVT. Specifically, we present extended dataset samples from roadside infrastructure in Fig.~\ref{fig:pose_variation}. In Fig.~\ref{fig:additional_variations}, we present with additional extended dataset samples for additional types of data variations due to varing weather and light conditions. 





==> sections/08_BEVT.tex <==
\section{BEVT Implementation}

\setlength{\tabcolsep}{3pt}
\begin{table*}[h!]
\centering
\fontsize{9}{12}\selectfont
%\bgroup\footnotesize
\begin{threeparttable}
\caption{}
\label{table:data_sensor}
\begin{tabular}{C{3cm}|C{6cm}C{2cm}}
\toprule %%%%%%%%%%%%%%%%%%
& Size & \\
\midrule
\midrule
\multirow{3}{*}{Image Encoder} & $L_k \times 64 \times 64 \times 128$ &  \\
& $L_k \times 32 \times 32 \times 256$ &  \\
& $L_k \times 16 \times 16 \times 512$ &  \\
Positional Encoder &  & \\
BEV Encoder & 128 128 128 & \\
Transformer &  & \\
BEV Decoder &  & \\

\bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\end{threeparttable}
\end{table*}

==> sections/09_ablation_study.tex <==
\section{Effectiveness}

To confirm that (\emph{i}) the differences between the data we proposed lead to variations in model training outcomes, and (\emph{ii}) personalized FedBEVT is effective in addressing these differences, we conducted ablation experiments using UC1 as an example to train models for different clients.

We first train models using only local data and tested them on various clients. In particular, we train a model using virtual car client with OPV2V~\cite{xu2022opv2v} data. Although it achieves an IoU of 30.48\% on car client data, its performance significantly decreased on the bus and truck testsets (7.39\% and 2.01\%), and it even performs worse than models trained using local truck data on the truck testset. This motivates us to use FedBEVT.

Subsequently, we employ different personalized FedBEVT, namely FedTP~\cite{li2022fedtp}, FedReg~\cite{collins2021exploiting}, and FedCaP, to train models for different clients and evaluate them on their own testsets and the testsets of other clients. The results shown in Tab.~\ref{table:AB_FedTP}, Tab.~\ref{table:AB_FedReg} and Tab.~\ref{table:AB_FedCaP} are consistent, with only locally personalized models being the most suitable for local data. Since the camera pose and quantity of a car typically do not change once it is produced, the locally collected training dataset and the data used for future inference have strong similarities. This aligns with our experimental design. Therefore, these results further emphasize the significance of personalized FedBEVT for road traffic perception in BEV.


\setlength{\tabcolsep}{3pt}
\begin{table}[h!]
\centering
\fontsize{8}{12}\selectfont
%\bgroup\footnotesize
\begin{threeparttable}
\caption{The BEVT model trained on local dataset and OPV2V dataset cannot well perform on local test dataset, which motivates to train with FedBEVT}
\label{table:uc4}
\begin{tabular}{C{3.5cm}|C{1.2cm}C{1.2cm}}
\toprule %%%%%%%%%%%%%%%%%%
\backslashbox{Local Testset}{ Trainset}&\multicolumn{1}{c}{Local} & \multicolumn{1}{c}{OPV2V}\\
\midrule
\midrule
Bus client & 5.42\% & 7.39\% \\
\midrule
Truck client& 4.16\% & 2.01\% \\
\bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\end{threeparttable}
\end{table}


\setlength{\tabcolsep}{3pt}
\begin{table}[h!]
\centering
\fontsize{8}{12}\selectfont
%\bgroup\footnotesize
\begin{threeparttable}
\caption{Average IoU of BEV detection for each client using personalized models trained with FedTP.}
\label{table:AB_FedTP}
\begin{tabular}{C{3.5cm}|C{1.2cm}C{1.2cm}C{1.2cm}}
\toprule %%%%%%%%%%%%%%%%%%
\backslashbox{Local Testset}{Per. Model}&\multicolumn{1}{c}{Bus client} & \multicolumn{1}{c}{Truck client} & \multicolumn{1}{c}{Car client}\\
\midrule
\midrule
Bus client & \textbf{10.72\%} &  4.61\%  & 9.12\% \\
\midrule
Truck client & 6.92\%  & \textbf{8.82\%} &  2.10\% \\
\midrule
Car client & 12.45\% &  6.76\% & \textbf{33.50\%} \\
\bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\end{threeparttable}
\end{table}



\setlength{\tabcolsep}{3pt}
\begin{table}[h!]
\centering
\fontsize{8}{12}\selectfont
%\bgroup\footnotesize
\begin{threeparttable}
\caption{Average IoU of BEV detection for each client using personalized models trained with FedReg.}
\label{table:AB_FedReg}
\begin{tabular}{C{3.5cm}|C{1.2cm}C{1.2cm}C{1.2cm}}
\toprule %%%%%%%%%%%%%%%%%%
\backslashbox{Local Testset}{Per. Model}&\multicolumn{1}{c}{Bus client} & \multicolumn{1}{c}{Truck client} & \multicolumn{1}{c}{Car client}\\
% \cmidrule(lr{0em}){2-10}
%& Train Loss & Avg. IoU & Comm. &  Train Loss & Avg. IoU & Comm. & Train Loss & Avg. IoU & Comm.\\
\midrule
\midrule
Bus client & \textbf{19.40\%} &  17.73\%  & 9.39\%\\
\midrule
Truck client & 9.59\%  & \textbf{14.20\%} &  4.48\% \\
\midrule
Car client & 26.04\%  &  20.39\% & \textbf{34.37\%} \\
\bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\end{threeparttable}
\end{table}

\setlength{\tabcolsep}{3pt}
\begin{table}[h!]
\centering
\fontsize{8}{12}\selectfont
%\bgroup\footnotesize
\begin{threeparttable}
\caption{Average IoU of BEV detection for each client using personalized models trained with FedCaP.}
\label{table:AB_FedCaP}
\begin{tabular}{C{3.5cm}|C{1.2cm}C{1.2cm}C{1.2cm}}
\toprule %%%%%%%%%%%%%%%%%%
\backslashbox{Local Testset}{Per. Model}&\multicolumn{1}{c}{Bus client} & \multicolumn{1}{c}{Truck client} & \multicolumn{1}{c}{Car client}\\
\midrule
\midrule
Bus client & \textbf{19.32\%} &  17.48\%  & 13.71\%\\
\midrule
Truck client & 13.01\%  & \textbf{15.01\%} &  8.89 \\
\midrule
Car client & 26.94\% & 25.26\%  & \textbf{35.44\%} \\
\bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\end{threeparttable}
\end{table}







==> sections/10_networks.tex <==
\section{Performance in Heterogeneous Networks}


\begin{figure*}[!ht]
\centering
\begin{subfigure}[b]{1\textwidth}
  \includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/FedBEVT_Networks_Dataset.png}
   \caption{Distribution of federated dataset with 58 clients for evaluation of FedBEVT under network assumption.}
   \label{fig:network1}
   \vspace{0.5cm}
\end{subfigure}

\begin{subfigure}[b]{1\textwidth}
   \includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/FedBEVT_Networks.png}
   \caption{Test Results on local test data from bus, truck, and car client respectively.}
   \label{fig:network2} 
\end{subfigure}
\caption{Exploring the impact of stragglers on the performance of FedBEVT in a challenging use case (UC5) with 58 connecting vehicle clients}
\label{fig:network}
\end{figure*}


Federated learning is often based on the fundamental assumption of network heterogeneity~\cite{li2020federated, wang2020tackling,karimireddy2020scaffold}, which is often observed in large-scale distributed wireless communication scenarios~\cite{li2023mocosfl, 9922064}. This is particularly relevant when using mobile devices such as phones and tablets for federated learning. In our use case, we are applying federated learning to intelligent transportation systems, where clients' data comes from private sources like OEMs and Tier-1s. In this context, the learning process typically occurs in a stable network environment, as clients have adequate communication resources. Therefore, data heterogeneity, not network heterogeneity, is the primary concern.

However, in federated learning organized in public traffic, where every car can exchange models with the server via wireless vehicular networks, network heterogeneity needs to be considered. To address this scenario, we have designed a challenging use case (UC~5) to validate the performance of FedBEVT in various network environments. Specifically, we have distributed the data to 58 vehicle clients, each with only one scenario, and included some stragglers in each communication round, as shown in~\ref{fig:network1}. Note that stragglers are clients with poor network communication environments who cannot upload their local updated model promptly, thereby losing the opportunity to contribute to the global model.

We have demonstrated the performance of FedBEVT (with FedAvg) under different straggler ratios of 0\%, 20\%, 40\%, 60\%, and 80\%. Fig.~\ref{fig:network2} shows the reduction of IoU affected by increasing ratio of stragglers.

==> sections/11_comm_comp.tex <==
\section{Communication Efficiency}

In federated learning scenarios, communication is typically considered a highly expensive resource, often even more so than computation resources~\cite{mcmahan2017communication, wang2022communication,wu2022communication}. As a result, improving communication efficiency is a critical research direction. One effective approach for improving communication efficiency is to increase the number of local training epochs, even though this may lead to higher computational costs. By doing so, each client can train more extensively on their local data before each communication round. In this study, we conduct experiments to investigate the impact of different numbers of local epochs on the performance of FedBEVT in UC~2, using two dedicated communication volumes (15 and 30 Gigabit). As shown in Fig.~\ref{fig:epoch}, our results indicate that a relatively large number of local epochs (e.g., 10 epochs per communication round) can generally increase the average IoU in most clients. However, we also observe that the impact of a large epoch number varied across clients, and in some cases (e.g., for the Truck client), it even lead to worse results due to local over-fitting. This observation is consistent with previous research on federated transformer learning~\cite{qu2022rethinking}.

\begin{figure}[t!]
   \centering
   \includegraphics[width=0.5\textwidth]{figures/FedBEVT_epochs.png}
   \caption{Exploring the impact of local epoch numbers on the performance of FedBEVT in UC~2 with a dedicated communication volume (CV) (left: 15~Gigabits, right: 30~Gigabits). }
   \label{fig:epoch}
\end{figure}

==> sections/12_further_visual_res.tex <==
\section{Further Visual Results}

We provide further visual comparisons of FedCaP against other federated learning methods in Fig.~\ref{fig:vis_bus},~Fig.~\ref{fig:vis_truck}, and Fig.~\ref{fig:vis_car} for bus, truck, and car, respectively. The qualitative results demonstrate that FedCaP outperforms other baseline methods in various road scenarios.


\begin{figure*}[!ht]
   \centering   \includegraphics[width=1\textwidth]{figures/further_vis_bus.png}
   \caption{Further visual results of FedCaP and other baselines on test data in a bus client.}
   \label{fig:vis_bus}
\end{figure*}

\begin{figure*}[!ht]
   \centering   \includegraphics[width=1\textwidth]{figures/further_vis_truck.png}
   \caption{Further visual results of FedCaP and other baselines on test data in a truck client.}
   \label{fig:vis_truck}
\end{figure*}

\begin{figure*}[!ht]
   \centering   \includegraphics[width=1\textwidth]{figures/further_vis_car.png}
   \caption{Further visual results of FedCaP and other baselines on test data in a car client.}
   \label{fig:vis_car}
\end{figure*}

==> sections/13_checklist.tex <==
\section{The Machine Learning Reproducibility Checklist}
\mypara {For all models and algorithms presented, check if you include:}

\mycheck ~~A clear description of the mathematical setting, algorithm, and/or model.

\mycheck ~~A clear explanation of any assumptions.

\mycheck ~~An analysis of the complexity (time, space, sample size) of any algorithm.

\mypara {For any theoretical claim, check if you include:}

\myuncheck ~~A clear statement of the claim.

\myuncheck ~~A complete proof of the claim.

\mypara {For all datasets used, check if you include:}

\mycheck ~~The relevant statistics, such as number of examples.

\mycheck ~~The details of train / validation / test splits.

\mycheck ~~An explanation of any data that were excluded, and all pre-processing step.

\mycheck ~~A link to a downloadable version of the dataset or simulation environment.

\mycheck ~~For new data collected, a complete description of the data collection process, such as instructions to annotators and methods for quality control.

\mypara {For all shared code related to this work, check if you include:}

\mycheck ~~Specification of dependencies.

\mycheck ~~Training code.

\mycheck ~~Evaluation code.

\mycheck ~~(Pre-)trained model(s).

\mycheck ~~README file includes table of results accompanied by precise command to run to produce those results.

\mypara {For all reported experimental results, check if you include:}

\mycheck ~~The range of hyper-parameters considered, method to select the best hyper-parameter configuration, and specification of all hyper-parameters used to generate results.

\mycheck ~~The exact number of training and evaluation runs.

\mycheck ~~A clear definition of the specific measure or statistics used to report results.

\mycheck ~~A description of results with central tendency (e.g. mean) \& variation (e.g. error bars).

\mycheck ~~The average runtime for each result, or estimated energy cost.

\mycheck ~~A description of the computing infrastructure used.
